Taguchi based Design of Sequential Convolution Neural Network for Classification of Defective Fasteners

Fasteners play a critical role in securing various parts of machinery. Deformations such as dents, cracks, and scratches on the surface of fasteners are caused by material properties and incorrect handling of equipment during production processes. As a result, quality control is required to ensure safe and reliable operations. The existing defect inspection method relies on manual examination, which consumes a significant amount of time, money, and other resources; also, accuracy cannot be guaranteed due to human error. Automatic defect detection systems have proven impactful over the manual inspection technique for defect analysis. However, computational techniques such as convolutional neural networks (CNN) and deep learning-based approaches are evolutionary methods. By carefully selecting the design parameter values, the full potential of CNN can be realised. Using Taguchi-based design of experiments and analysis, an attempt has been made to develop a robust automatic system in this study. The dataset used to train the system has been created manually for M14 size nuts having two labeled classes: Defective and Non-defective. There are a total of 264 images in the dataset. The proposed sequential CNN comes up with a 96.3% validation accuracy, 0.277 validation loss at 0.001 learning rate.

==> mybibliography.tex <==
@article{Yun2009,
	affiliation = {Electrical and Computer Engineering Division, Pohang University of Science and Technology (POSTECH), Pohang 790-784, Republic of Korea; Department of Electronics Engineering, Dong-A University, Busan 604-714, Republic of Korea},
	author = {Yun, Jong Pil and Choi, SungHoo and Kim, Jong-Wook and Kim, Sang Woo},
	doi = {10.1016/j.ndteint.2009.01.007},
	journal = {NDT and E International},
	keywords = {Defect detection; Vision inspection; Surface flaw; Gabor filter; uDEAS},
	language = {English},
	number = {5},
	pages = {389-397},
	title = {Automatic detection of cracks in raw steel block using Gabor filter optimized by univariate dynamic encoding algorithm for searches (uDEAS)},
	volume = {42},
	year = {2009},
}
@article{chen2017automatic,
  title={Automatic defect detection of fasteners on the catenary support device using deep convolutional neural network},
  author={Chen, Junwen and Liu, Zhigang and Wang, Hongrui and N{\'u}{\~n}ez, Alfredo and Han, Zhiwei},
  journal={IEEE Transactions on Instrumentation and Measurement},
  volume={67},
  number={2},
  pages={257--269},
  year={2017},
  publisher={IEEE}
}
@inproceedings{saiz2018robust,
  title={A robust and fast deep learning-based method for defect classification in steel surfaces},
  author={Saiz, F{\'a}tima A and Serrano, Ismael and Barandiar{\'a}n, I{\~n}igo and S{\'a}nchez, Jairo R},
  booktitle={2018 International Conference on Intelligent Systems (IS)},
  pages={455--460},
  year={2018},
  organization={IEEE}
}
@inproceedings{sharifzadeh2008detection,
  title={Detection of steel defect using the image processing algorithms},
  author={Sharifzadeh, M and Amirfattahi, R and Sadri, S and Alirezaee, S and Ahmadi, M},
  booktitle={The International Conference on Electrical Engineering},
  volume={6},
  number={6th International Conference on Electrical Engineering ICEENG 2008},
  pages={1--7},
  year={2008},
  organization={Military Technical College}
}
@article{xue2021key,
  title={Key Technologies of Steel Plate Surface Defect Detection System Based on Artificial Intelligence Machine Vision},
  author={Xue, Bin and Wu, Zhisheng},
  journal={Wireless Communications and Mobile Computing},
  volume={2021},
  year={2021},
  publisher={Hindawi}
}
@article{xue2021detection,
  title={Detection of Various Types of Metal Surface Defects Based on Image Processing.},
  author={Xue, Peng and Jiang, Changhong and Pang, Huanli},
  journal={Traitement du Signal},
  volume={38},
  number={4},
  year={2021}
}
@article{mohan2018crack,
  title={Crack detection using image processing: A critical review and analysis},
  author={Mohan, Arun and Poobal, Sumathi},
  journal={Alexandria Engineering Journal},
  volume={57},
  number={2},
  pages={787--798},
  year={2018},
  publisher={Elsevier}
}
@inproceedings{caleb2000classification,
  title={Classification of surface defects on hot rolled steel using adaptive learning methods},
  author={Caleb, P and Steuer, M},
  booktitle={KES'2000. Fourth International Conference on Knowledge-Based Intelligent Engineering Systems and Allied Technologies. Proceedings (Cat. No. 00TH8516)},
  volume={1},
  pages={103--108},
  year={2000},
  organization={IEEE}
}
@article{ashour2015texture,
  title={Texture-based classification of workpiece surface images using the support vector machine},
  author={Ashour, Mohammed Waleed and Halin, Alfian Abdul and Khalid, Fatimah and Abdullah, Lili Nurliyana and Darwish, Samy H},
  journal={International Journal of Software Engineering and Its Applications},
  volume={9},
  number={10},
  pages={147--160},
  year={2015}
}
@article{park2016machine,
  title={Machine learning-based imaging system for surface defect inspection},
  author={Park, Je-Kang and Kwon, Bae-Keun and Park, Jun-Hyub and Kang, Dong-Joong},
  journal={International Journal of Precision Engineering and Manufacturing-Green Technology},
  volume={3},
  number={3},
  pages={303--310},
  year={2016},
  publisher={Springer}
}
@book{taguchi1,
  title={A first course in design and analysis of experiments},
  author={Oehlert, Gary W},
  year={2010}
}
@book{mont1,
  title={Design and analysis of experiments},
  author={Montgomery, Douglas C},
  year={2017},
  publisher={John wiley \& sons}
}
